SECTOR: A Neural Model for Coherent Topic Segmentation and Classification

When searching for information, a human reader first glances over a document, spots relevant sections and then focuses on a few sentences for resolving her intention. However, the high variance of document structure complicates to identify the salient topic of a given section at a glance. To tackle this challenge, we present SECTOR, a model to support machine reading systems by segmenting documents into coherent sections and assigning topic labels to each section. Our deep neural network architecture learns a latent topic embedding over the course of a document. This can be leveraged to classify local topics from plain text and segment a document at topic shifts. In addition, we contribute WikiSection, a publicly available dataset with 242k labeled sections in English and German from two distinct domains: diseases and cities. From our extensive evaluation of 20 architectures, we report a highest score of 71.6% F1 for the segmentation and classification of 30 topics from the English city domain, scored by our SECTOR LSTM model with bloom filter embeddings and bidirectional segmentation. This is a significant improvement of 29.5 points F1 compared to state-of-the-art CNN classifiers with baseline segmentation.

==> table_classes.tex <==
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{en\_disease (27)} & \textbf{de\_disease (25)} & \textbf{en\_city (30)}      & \textbf{de\_city (27)}     \\ \midrule
treatment            & therapie             & history                & geschichte            \\
symptom              & diagnose             & demography             & geographie            \\
diagnosis            & symptom              & geography              & verkehr               \\
cause                & ursache              & education              & tourismus             \\
classification       & kategorisierung      & culture                & demografie            \\
epidemiology         & verlauf              & transport              & gemeinde              \\
history              & epidemiologie        & economics              & wirtschaft            \\
prognosis            & geschichte           & politics               & kultur                \\
management           & prognose             & climate                & bildung               \\
pathophysiology      & praevalenz           & sport                  & politik               \\
mechanism            & vorbeugung           & district               & infrastruktur         \\
prevention           & fauna                & media                  & regierung             \\
research             & terminologie         & sights                 & sport                 \\
genetics             & pathologie           & international\_affairs & gemeindepartnerschaft \\
tomography           & definition           & environment            & religion              \\
culture              & klinik               & etymology              & menschen              \\
etymology            & komplikation         & tourism                & etymologie            \\
infection            & genetik              & infrastructure         & kirche                \\
fauna                & infektion            & recreation             & stadtlandschaft       \\
risk                 & risiko               & facility               & klima                 \\
pathology            & forschung            & people                 & presse                \\
surgery              & geographie           & architecture           & architektur           \\
screening            & mensch               & society                & kriminalitaet         \\
medication           & organe               & faith                  & ueberblick            \\
geography            & sonstiges            & health                 & erholung              \\
complication         &                      & overview               & stadtviertel          \\
other                &                      & science                & sonstiges             \\
                     &                      & law                    &                       \\
                     &                      & crime                  &                       \\
                     &                      & other                  &                       \\ \bottomrule
\end{tabular}

